Kernel Density Estimation based Factored Relevance Model for Multi-Contextual Point-of-Interest Recommendation

An automated contextual suggestion algorithm is likely to recommend contextually appropriate and personalized 'points-of-interest' (POIs) to a user, if it can extract information from the user's preference history (exploitation) and effectively blend it with the user's current contextual information (exploration) to predict a POI's 'appropriateness' in the current context. To balance this trade-off between exploitation and exploration, we propose an unsupervised, generic framework involving a factored relevance model (FRLM), constituting two distinct components, one pertaining to historical contexts, and the other corresponding to the current context. We further generalize the proposed FRLM by incorporating the semantic relationships between terms in POI descriptors using kernel density estimation (KDE) on embedded word vectors. Additionally, we show that trip-qualifiers, (e.g. 'trip-type', 'accompanied-by') are potentially useful information sources that could be used to improve the recommendation effectiveness. Using such information is not straight forward since users' texts/reviews of visited POIs typically do not explicitly contain such annotations. We undertake a weakly supervised approach to predict the associations between the review-texts in a user profile and the likely trip contexts. Our experiments, conducted on the TREC contextual suggestion 2016 dataset, demonstrate that factorization, KDE-based generalizations, and trip-qualifier enriched contexts of the relevance model improve POI recommendation.

==> sections/algo.tex <==
%\para{Generic Overview}
In this section, we present the algorithmic details of our proposed models.
To summarize, referring back to Figure \ref{fig:frlm}, our proposed approach needs estimating a total of three relevance models. First, the relevance model based on a user's profile information, $\theta_{U, q_U}$, is estimated (with or without applying the kernel function based density estimation) by making use of the tags and text present in a user's profile. Next, to capture the appropriateness of POIs in a \emph{hard} contextual constraint (current location), we estimate the factored RLM $\theta_{U, q_U, l_U}$ by making use of information from both the user profile and the top ranked POIs in the current location, considering the former as analogous to a query and the latter as pseudo-relevant documents, again with or without the kernel factor.
%within an RLM set up \cite{Lavrenko_RLM2001:RBL:383952.383972}.
Finally, these two relevance models $\theta_{U, q_U}$ and $\theta_{U, q_U, l_U}$ are merged into a combined relevance model $\theta$, using a linear combination.
%, the proposed generalized FRLM or KDEFRLM.

% While estimating $\theta_U$ is similar to the traditional RLM \cite{Lavrenko_RLM2001:RBL:383952.383972} in IR, our underlying assumption is that both `tags', those given by a user and those extracted from the POIs rated by that user, are sampled from a latent relevance model $\theta_U$. More formally, for a user $U$, set of tuple $P_i$'s $= (D, T, r) \in U$ are considered as the set of (pseudo-)relevant POIs and the set of `tags' from the set of tuples $(D, T, r)$ is the absolute evidence about $\theta_U$.
%While estimating $\theta_U$, similar to the traditional RLM \cite{Lavrenko_RLM2001:RBL:383952.383972} in IR, our underlying assumption is that both `tags', given by a user and the (document representation of) POIs in preference history, rated by that user are sampled from a latent relevance model $\theta_U$. More formally, for a user $U$, set of tuple $P_i$'s $= (D, T, r) \in U$ are considered as the set of (pseudo-)relevant POIs and the set of `tags' from the set of tuples $(D, T, r)$ is the absolute evidence about $\theta_U$.

%On the other hand, Factored RLM $\theta_{U, C(U)}$ for contextual relevance is estimated in the same way, but here the set of top retrieved POIs are considered as the set of (pseudo-)relevant POIs and the estimated user profile based relevance model $\theta_U$ itself is the absolute evidence about the relevance model $\theta_{U, C(U)}$.


\input{tables/algo}


%\subsection{Proposed Algorithm} \label{Algorithm}

\para{Initialization}
As shown in Algorithm \ref{Algorithm:PseudoCode}, let a user profile is presented as $U = \cup_{i=1}^{N_U} \{P_i: P_i = (D, T, r)\}$ (Equation \ref{eq:profile}), along with $q_U$, as the \emph{soft} contextual constraint and $l_U$, as the \emph{hard} location constraint. We define $T'$, as the set of user assigned (unique) tags i.e. union of all $T$s from the set of tuples $(D, T, r) \in U$ and $M_U$, as the union of all documents, $D$s from the set of tuples $(D, T, r) \in U$. We then perform an initial retrieval to get a set of top retrieved documents, $M_{l_U}$, while queried with the set of tags, $T'$. Please note that, this is an example of a constrained retrieval, i.e the retrieved documents in $M_{l_U}$, are the documents constrained to the \emph{hard} location constraint $l_U$.

In addition, we create a vector representation,
%$\mathcal{D}_{vec}$,
for all terms in the static collection $\mathcal{D}$, using $word2vec$ \cite{Word2vec_NIPS2013}. While training $word2vec$, we set the size of word vectors as $200$, maximum skip length between words as $8$, number of negative samples as $25$, threshold for occurrence of words as $1e-4$, number of threads as $20$, number of training iterations as $15$ and use the continuous bag-of-words model.


\para{Estimate User Profile Based RLM}
After the initialization step, we estimate the factor model $\theta_{U, q_U}$, which is a relevance model based on user profile information. For each term $w \in M_U$, we estimate $P(w|\theta_{U, q_U})$, i.e. the probability of sampling the term $w$ from the relevance model $\theta_{U, q_U}$ (Equation \ref{eq:kderlmprofile}). Note that, it is essentially done by the joint probability of observing the term $w$, along with the user assigned tags, $T'$, with the help of KDE. As we mentioned earlier, that we apply the multiplicative semantic evidence approach for KDE while estimating the user profile based RLM, as it performed better than the generalized KDE approach.

Note that, the estimation of the relevance model is in fact a mixture model of the estimated model $\theta_{U, q_U}$ in conjunction with $P(w|T')$, the tag likelihood model, to get the influence of the user assigned tags $T'$, in the actual estimation of $\theta_{U, q_U}$. We use maximum likelihood estimation (MLE) to compute the tag likelihood model, $P(w|T')$. $\mu_U$ acts as a smoothing (tag mixing) parameter to control the relative weight we set to the relevance model itself versus the tag model. From the mixture model, we get the actual probability of the term $w$, $P'(w|\theta_{U, q_U})$. Now the probability $P'(w|\theta_{U, q_U})$, along with the actual term $w$, are stored in an initially empty list, $L_U$. Note that, the term itself and its probability are stored as a single entity, $\{w, P'(w|\theta_{U, q_U})\}$, in the list. Once we are finished computing the probability of every term in $M_U$, we sort the list $L_U$, in decreasing order of the probability value $P'(w|\theta_{U, q_U}$. Top $\tau$ terms are then extracted from $L_U$, and added to another initially empty list, $L'_U$ (along with their associated $P'(w|\theta_{U, q_U})$ values).


\para{Estimate Factored RLM}
After estimating the first relevance model (the factor model), we estimate the factored relevance model, $\theta_{U, q_U, l_U}$, from the set of documents, $M_{l_U}$, in the similar way. As shown in Algorithm \ref{Algorithm:PseudoCode}, this time we compute the probability of sampling a term $w$, $P(w|\theta_{U, q_U, l_U})$ by the joint probability of observing the term $w$, along with the set of terms estimated in the former user profile based relevance model, $\theta_{U, q_U}$, again with the help of KDE (Equation \ref{eq:kdeflm}). This time we followed the generalized semantic evidence approach for KDE, as it performed better than the multiplicative KDE approach. We create a list of terms (along with their associated $P'(w|\theta_{U, q_U, l_U})$ values), $L'_{l_U}$ in the similar fashion we created $L'_U$.


\para{Generalization of FRLM}
We then combine these two lists, $L'_U$, and $L'_{l_U}$ into a final list, $L$, using a linear combination (Equation \ref{eq:frlm_linearcomb}), where $\gamma_H$ acts as the trade-off parameter to balance \emph{exploitation-exploration}. We define $T''$, as a weighted term distribution by extracting the set of all terms from the list, $L$, where the weight of each term is the corresponding probability of that term in $L$. This term distribution, $T''$ can be considered analogous to expanded query of the original query, $T'$. Now, we perform the final constrained (to the \emph{hard} location constraint, $l_U$) retrieval, using $T''$ as the query, to generate the final rank list of documents (POIs) for the user $U$.


Note that, based on the way we compute $P(w|\theta_{U, q_U})$ and $P(w|\theta_{U, q_U, l_U})$, we report the results of two variations of our proposed model. The result of our proposed approach is denoted by `FRLM', when $P(w|\theta_{U, q_U})$ and $P(w|\theta_{U, q_U, l_U})$ are computed based on Equation \ref{eq:rlmprofile} and \ref{eq:flm}, respectively. On the other hand, we refer to the result of our proposed approach as `KDEFRLM', when $P(w|\theta_{U, q_U})$ and $P(w|\theta_{U, q_U, l_U})$ are computed based on Equation \ref{eq:kderlmprofile} and \ref{eq:kdeflm}, respectively.







==> sections/background.tex <==
\section{Background}
In this section we briefly outline Kernel Density Estimation (KDE), a statistical technique to estimate a probability distribution, which we use in our proposed relevance feedback model. We then provide a general description of the relevance model (RLM), which is a pseudo-relevance feedback method, followed by a short review of a generalized KDE based RLM method, underlying theory of which is applicable to our proposed model.

\subsection{Kernel Density Estimation}
Kernel Density Estimation (KDE) is a non-parametric method to estimate the probability density function of a random variable. Formally, let $\{x_1, \dots, x_n\}$ be independent and identically distributed (i.i.d.) samples drawn from a distribution. The shape of the density function $f$, from which these points are sampled can be estimated as in Equation \ref{eq:weightedKDE}.
\begin{equation} \label{eq:weightedKDE}
	\hat f_\alpha(x) = \frac{1}{nh} \sum_{i=1}^n \alpha_i K \Big(\frac{x-x_i}{h}\Big)
\end{equation}
In Equation \ref{eq:weightedKDE}, $\hat f_\alpha(x)$ is the estimated value of the true density function $f(x)$, where $K(.)$ is a kernel function scaled by a bandwidth parameter $h$. Please note that Equation \ref{eq:weightedKDE} is a generalized weighted version of KDE in which the kernel function around the $i^{th}$ data point is weighted by $\alpha_i$, where $\sum_i \alpha_i = 1$.



\subsection{Relevance Model for IR} \label{RelevanceModelRevisited}
%The main hypothesis of the relevance model \cite{Lavrenko:2001:RBL:383952.383972} (RLM) is that both a query and the relevant documents of that query are sampled from a latent relevance model \textit{R}, that needs to be estimated. Traditionally top retrieved documents are considered as the set of (pseudo-)relevant documents \textit{M} and the query $Q = \{q_1, ..., q_k\}$  is the absolute evidence about \textit{R}. The probability of sampling a term \textit{w} from \textit{R}, denoted by $P(w|R)$ is approximated as in Equation \ref{eq:JointProbability} by the joint probability of observing \textit{w} along with the query terms $q_1, ..., q_k$.
The traditional relevance model (RLM) \cite{Lavrenko_RLM2001:RBL:383952.383972} is a relevance feedback technique which estimates terms' importance for relevance feedback by using the co-occurrence information between a set of given query terms and the ones in a set of top-retrieved documents. According to the underlying theory, RLM assumes that the terms frequently co-occurring with the query terms are semantically related to the actual information need and, therefore, could be useful to enrich the query with additional information.

Formally speaking, given a query $Q=\{q_1,\ldots,q_n\}$, RLM essentially estimates a term weight distribution $P(w|Q)$ from a set of $M$ top-retrieved documents $\mathcal{M}=\{D_1,\ldots,D_M\}$, i.e.,
\begin{equation} \label{eq:traditional_rlm}
	P(w|Q) = \sum_{D \in \mathcal{M}} P(w|D) \prod_{q \in Q} P(q|D).
\end{equation}
Intuitively, it can be seen that higher $P(w|Q)$ values (RLM term weights) are achieved for a term $w$ if it occurs frequently in a top-retrieved document (large $P(w|D)$ value), in conjunction with the frequent occurrence of a query term $q \in Q$ such that $P(q|D)$ is also large.


\subsection{Kernel Density Estimation Based RLM}
Roy et al. \cite{DoiKDERLM_CIKM16} introduced semantic relationships between terms, along with document-level co-occurrence of terms, for better estimation of $P(w|Q)$. With the query terms $Q = \{q_1, \dots, q_n\}$ embedded as vectors, the probability density function has been estimated with KDE as shown in Equation \ref{eq:KDERLM_1D}. More formally,
\begin{equation} \label{eq:KDERLM_1D}
    f(w) = \frac{1}{nh} \sum_{i=1}^n P(w|\mathcal{M}) P(q_i|\mathcal{M}) K \Big(\frac{w-q_i}{h}\Big),
    %f(w) = \sum_{i=1}^k P(w|\mathcal{M}) P(q_i|\mathcal{M}) \frac{1}{\sigma \sqrt{2 \pi}} exp (-\frac{(w-q_i)^T (w-q_i)}{2\sigma^2 h^2}),
\end{equation}
where the applied kernel function $K(.)$ is a Gaussian one with the weight around the $i^{th}$ data point is considered as $P(w|\mathcal{M}) P(q_i|\mathcal{M})$, $\mathcal{M}$ being the set of terms in top ranked documents. i.e. for a candidate term $w$, the (semantically) closer $w$ is to a query term $q_i$, along with the higher RLM term weights, the higher is the value of the density function $f(w)$.


==> tables/algo.tex <==
\begin{algorithm}[htb]
\small
%\begin{algorithm}[]
\SetAlgoLined

%\KwResult{Write here the result }

%Set $\mathcal{U} \gets$ User requests
\textbf{Input:} $U$, $q_U$, $l_U$, $\mu_U$, $\mu_{l_U}$, $\tau$, $\gamma_H$\\
%, $\mathcal{D}_{vec}$\\
\textbf{Output:} List of POIs\\
%\While{$U = \cup_{i=1}^{N_U} \{P_i: P_i = (D, T, r)\} \in \mathcal{U}$}{
    \tcp{Initialization}
    $T' \gets$ Union of all $T$s $\in U = \cup_{i=1}^{N_U} \{P_i: P_i = (D, T, r)\}$ %where $r \geq 0.8$
    \tcp{user assigned tags}
    $M_U \gets$ Union of all $D$s $\in U = \cup_{i=1}^{N_U} \{P_i: P_i = (D, T, r)\}$ %where $r \geq 0.8$ 
    \tcp{documents in user's pref. history}
    %$M_{l_U} \gets$ Top $M$ documents from retrieve($T'$, $l_U$) \tcp{top-ranked POIs, constrained to location $l_U$}
    $M_{l_U} \gets retrieve(T', l_U)$ \tcp{top retrieved documents, constrained to location $l_U$, while queried with $T'$}
    %$n \gets |T'|$ \tcp{no. of terms in $T'$}
    %\vspace{10pt}
    \tcp{Exploitation: Estimate relevance model $\theta_{U, q_U}$ from $M_{U}$}
    $i=0, L_U \gets null, L'_U \gets null$\\
    \For{each term $w \in M_U$} {
        $wVec \gets getVector(w)$ \tcp{get vector for $w$}% from $\mathcal{D}_{vec}$}
        %$P(w|\theta_U) = \sum_{(D,T,r) \in U} r P(w|D) \prod_{t \in T'}P(t|D)$
        $P(w|\theta_{U, q_U}) = 0$ \\
        \For{each $P_i = (D, T, r) \in U$} {
            $\kappa = 0$\\
            \For{each term $t \in T'$} {
                $tVec \gets getVector(t)$ \tcp{get vector for $t$}% from $\mathcal{D}_{vec}$}
                $dist \gets getEuclideanDist(wVec, tVec)$\\
                $\kappa \ +\!\!= \frac{1}{\sigma \sqrt{2 \pi}} exp (-\frac{dist}{2\sigma^2 h^2})$ \tcp{KDE score computation of term $t$}
            }
            %$P(w|\theta_{U, q_U}) \ +\!\!= r P(w|D) \psi(w, q_U) \big( \prod_{t \in T'} P(t|D) \big) \sum_{t \in T'} \frac{1}{\sigma \sqrt{2 \pi}} exp (-\frac{(\mathbf{w}-\mathbf{t})^T (\mathbf{w}-\mathbf{t})}{2\sigma^2 h^2})$
            $P(w|\theta_{U, q_U}) \ +\!\!= r P(w|D) \psi(w, q_U) \big( \prod_{t \in T'} P(t|D) \big) \kappa$
        }
        $P'(w|\theta_{U, q_U}) = \mu_U P(w|\theta_{U, q_U}) + (1-\mu_U) P(w|T')$\\
        $L_U[i+\!+] \gets \{w, P'(w|\theta_{U, q_U})\}$
    }
    Sort $L_U$ in descending order of $P'(w|\theta_{U, q_U})$\\
    $L'_U \gets$ top $\tau$ terms from $L_U$\\
    %$n_U \gets |L'_U|$ \tcp{no. of terms in $L'_U$}
    %\vspace{10pt}
    \tcp{Exploration: Estimate relevance model $\theta_{U, q_U, l_U}$ from $M_{l_U}$}
    $i=0, L_{l_U} \gets null, L'_{l_U} \gets null$\\
    \For{each term $w \in M_{l_U}$} {
        $wVec \gets getVector(w)$ \tcp{get vector for $w$}% from $\mathcal{D}_{vec}$}
        $P(w|\theta_{U, q_U, l_U}) = 0$ \\
        %$P(w|\theta_{U,C(U)}) = \sum_{d \in L(c)} P(w|d) \prod_{t \in \theta_U(w)} P(t|d)$
        \For{each term $t \in L'_U$} {
            $tVec \gets getVector(t)$ \tcp{get vector for $t$}% from $\mathcal{D}_{vec}$}
            $dist \gets getEuclideanDist(wVec, tVec)$\\
            $\kappa = \frac{1}{\sigma \sqrt{2 \pi}} exp (-\frac{dist}{2\sigma^2 h^2})$\\
            $P(w|\theta_{U, q_U, l_U}) \ +\!\!= P(w|M_{l_U}) P(t|M_{l_U}) \kappa$
        }
        %$P(w|\theta_{U,C(U)}) = \sum_{i=1}^{n_\theta} P(w|M_U) P(t_i|M_U) \frac{1}{\sigma \sqrt{2 \pi}} exp (-\frac{(\mathbf{w}-\mathbf{t_i})^T (\mathbf{w}-\mathbf{t_i})}{2\sigma^2 h^2})$
        $P'(w|\theta_{U, q_U, l_U}) = \mu_{l_U} P(w|\theta_{U, q_U, l_U}) + (1-\mu_{l_U}) P(w|\theta_{U, q_U})$\\
        $L_{l_U}[i+\!+] \gets \{w, P'(w|\theta_{U, q_U, l_U})\}$
    }
    Sort $L_{l_U}$ in descending order of $P'(w|\theta_{U, q_U, l_U})$\\
    $L'_{l_U} \gets$ top $\tau$ terms from $L_{l_U}$\\
    %\vspace{10pt}
    
%    \tcp{Re-ranking}
%    $M_R'$ $\gets$ $reRank_{KL-Div}$($M_R, P(w|\theta_{U,C(U)})$)\\
%    %SL: you state {KL-Div}$($M_R$) - but aren't you looping through and minimizing the divergence between a single item in M_R and $P(w|\theta_{R})$  
%    $P(w|\theta_{U,C(U)})$: Re-estimate $\theta_{U,C(U)}$ from $M_R'$\\
%    \vspace{10pt}

    \tcp{Estimate generalized KDE based factored relevance model $\theta$}
    $i=0, L \gets null$\\
    \For{each $w \in$ Union of ($L'_U, L'_{l_U})$}{
        %$P(w|\theta) = \gamma_H \cdot P'(w|\theta_U) + (1-\gamma_H) \cdot P'(w|\theta_{U,C(U)})$\\
        $P(w|\theta) = \gamma_H P(w|\theta_{U, q_U}) + (1-\gamma_H)P(w|\theta_{U, q_U, l_U})$\\
        $L[i+\!+] \gets \{w, P(w|\theta)\}$
    }
    %\vspace{10pt}
    
    \tcp{Query expansion}
    $T''$ $\gets$ all terms in $L$ \tcp{weighted term distribution}
    $retrieve(T'', l_U)$ \tcp{ranklist for $U$}
%}
\caption{Proposed Algorithm using KDEFRLM}
\label{Algorithm:PseudoCode}
\end{algorithm}


==> tables/resultsTable.tex <==
\begin{table}[htbp]
\centering
%\small
%\footnotesize
\caption{Comparisons between POI retrieval approaches.
%our proposed models and the other baseline methods investigated on both the location-only, $\psi_l$ (shaded with gray), and location plus trip qualifier, $\{\psi_s, \psi_j\}$, contexts.
The notations, `$^*$', `$^\dagger$' and `$^\ddagger$' denote significant (paired t-test with 95\% confidence) improvements over the three strongest baselines - BL5 (KDERLM), BL11 (Hybrid) and BL1 (BM25), respectively.}
\label{Table:ResultsCombined2}
\tabfitpagew
{
\begin{tabular}
    %{@{}lllllllllr@{}}
    {@{}l@{\ \ }l@{\ \ \ }l@{\ }l@{\ }l@{\ }ll@{\ }l@{\ }l@{\ \ }r@{}}
    \toprule
    & & Context & \multicolumn{3}{c}{Graded Evaluation Metrics} & \multicolumn{4}{c}{Binary Evaluation Metrics}\\
    \cmidrule(r){4-6}
    \cmidrule(l){7-10}
    \multicolumn{2}{c}{Method} & $(\psi)$ & nDCG@5 & nDCG@10 & nDCG & P@5 & P@10 & MAP & MRR \\
    \midrule
    \multicolumn{2}{c}{\textbf{IR-based approaches}} & & & & \\
    \midrule
    \rowcolor{lightgray}
    BL1 & BM25 & $\psi_l$ & 0.2747 & 0.2484 & 0.2889 & 0.3934 & 0.3066 & 0.1326 & 0.6539\\
    \multirow{2}{*}{BL1} & \multirow{2}{*}{BM25} & $\psi_s$ & 0.2609 & 0.2441 & 0.2889 & 0.3869 & 0.3164 & 0.1335 & 0.5967\\
    & & $\psi_j$ & 0.2641 & 0.2464 & 0.2916 & 0.3639 & 0.3033 & 0.1355 & 0.6565\\
    \rowcolor{lightgray}
    BL2 & Term Sel. & $\psi_l$ & 0.2484 & 0.2383 & 0.3034 & 0.3639 & 0.3066 & 0.1466 & 0.6148\\
    \multirow{2}{*}{BL2} & \multirow{2}{*}{Term Sel.} & $\psi_s$ & 0.2424 & 0.2411 & 0.3039 & 0.3607 & 0.3148 & 0.1458 & 0.6186\\
    & & $\psi_j$ & 0.2539 & 0.2447 & 0.3099 & 0.3705 & 0.3197 & 0.1514 & 0.6419\\
    \rowcolor{lightgray}
    BL3 & BM25 + Term Sel. & $\psi_l$ & 0.2411 & 0.2332 & 0.3143 & 0.3672 & 0.3115 & 0.1530 & 0.5607\\
    \multirow{2}{*}{BL3} & \multirow{2}{*}{BM25 + Term Sel.} & $\psi_s$ & 0.2462 & 0.2471 & 0.3207 & 0.3672 & 0.3344 & 0.1578 & 0.6095\\
    & & $\psi_j$ & 0.2530 & 0.2429 & 0.3195 & 0.3869 & 0.3328 & 0.1557 & 0.6191\\
    \rowcolor{lightgray}
    BL4 & RLM
    %\cite{Lavrenko_RLM2001:RBL:383952.383972}
    & $\psi_l$ & 0.2615 & 0.2453 & 0.3091 & 0.3574 & 0.3033 & 0.1437 & 0.6441\\
    \multirow{2}{*}{BL4} & \multirow{2}{*}{RLM}
    %\cite{Lavrenko_RLM2001:RBL:383952.383972}
    & $\psi_s$ & 0.2583 & 0.2466 & 0.3107 & 0.3475 & 0.3016 & 0.1443 & 0.6441\\
    & & $\psi_j$ & 0.2692 & 0.2514 & 0.3189 & 0.3639 & 0.3131 & 0.1496 & 0.6544\\
    \rowcolor{lightgray}
    BL5 & KDERLM
    %\cite{DoiKDERLM_CIKM16}
    & $\psi_l$ & 0.2829 & 0.2682 & 0.3191 & 0.3967 & 0.3361 & 0.1495 & 0.6539\\
    \multirow{2}{*}{BL5} & \multirow{2}{*}{KDERLM}
    %\cite{DoiKDERLM_CIKM16}
    & $\psi_s$ & 0.2839 & 0.2668 & 0.3236 & 0.3902 & 0.3902 & 0.1530 & 0.6639\\
    & & $\psi_j$ & 0.2772 & 0.2666 & 0.3287 & 0.3869 & 0.3311 & 0.1594 & 0.6623\\
    \midrule
    \multicolumn{2}{c}{\textbf{RecSys based approaches}} & & & & \\
    \midrule
    \rowcolor{lightgray}
    BL6 & Most Popular K & $\psi_l$ & 0.1861 & 0.1926 & 0.2580 & 0.2787 & 0.2705 & 0.1016 & 0.4154\\
    \multirow{2}{*}{BL6} & \multirow{2}{*}{Most Popular K} & $\psi_s$ & 0.1765 & 0.1894 & 0.2579 & 0.2590 & 0.2689 & 0.1015 & 0.4055\\
    & & $\psi_j$ & 0.1877 & 0.1844 & 0.2590 & 0.2656 & 0.2475 & 0.1010 & 0.4247\\
    \rowcolor{lightgray}
    BL7 & Profile Popular K & $\psi_l$ & 0.2488 & 0.2409 & 0.2811 & 0.3410 & 0.3016 & 0.1280 & 0.6486\\
    \multirow{2}{*}{BL7} & \multirow{2}{*}{Profile Popular K} & $\psi_s$ & 0.2529 & 0.2381 & 0.2861 & 0.3639 & 0.3016 & 0.1321 & 0.6296\\
    & & $\psi_j$ & 0.2568 & 0.2487 & 0.2908 & 0.3574 & 0.3098 & 0.1362 & 0.6500\\
    %\multirow{2}{*}{BL8:} & \multirow{2}{*}{PMF \cite{NMF_ProbabilisticMatrixFactorization}} & $N_c = 1$ & 0.2287 & 0.2169 & 0.2613 & 0.3443 & 0.2869 & 0.1165 & 0.5411\\
    %& & $N_c > 1$ &- & - & - & - & - & - & -\\
    \rowcolor{lightgray}
    BL8 & NeuMF
    %\cite{NCF_WWW2017}
    & $\psi_l$ & 0.1626 & 0.1655 & 0.2480 & 0.2361 & 0.2344 & 0.0937 & 0.4314\\
    \multirow{2}{*}{BL8} & \multirow{2}{*}{NeuMF}
    %\cite{NCF_WWW2017}
    & $\psi_s$ & 0.1491 & 0.1601 & 0.2466 & 0.2131 & 0.2344 & 0.0935 & 0.3969\\
    & & $\psi_j$ & 0.1698 & 0.1834 & 0.2457 & 0.2393 & 0.2525 & 0.0923 & 0.4300\\
    \rowcolor{lightgray}
    BL9 & Bayesian & $\psi_l$ & 0.2170 & 0.1774 & 0.1816 & 0.3082 & 0.2082 & 0.0672 & 0.5831\\
    %& & $N_c > 1$ & NA & NA & NA & NA & NA & NA & NA\\
    \midrule
    \multicolumn{2}{c}{\textbf{Hybrid approaches}} & & & & \\
    \midrule
    \rowcolor{lightgray}
    BL10 & Content + Tag.
    %\cite{Aliannejadi:2017:VAP:3077136.3080754}
    & $\psi_l$ & 0.2499 & 0.2411 & 0.2800 & 0.3967 & 0.3377 & 0.1330 & 0.5390\\
    \multirow{3}{*}{BL10} & \multirow{3}{*}{Content + Tag.}
    %\cite{Aliannejadi:2017:VAP:3077136.3080754}
    & $\psi_s$ & 0.2623 & 0.2496 & 0.2841 & 0.4066 & 0.3492 & 0.1383 & 0.5982\\
    & & $\psi_j$ & 0.2688 & 0.2651 & 0.2979 & 0.4000 & 0.3656 & 0.1484 & 0.6260\\
    & & SVM & 0.2656 & 0.2476 & 0.2833 & 0.3770 & 0.3262 & 0.1330 & 0.5850\\
    \rowcolor{lightgray}
    BL11 & Hybrid (BL5 + BL10) & $\psi_l$ & 0.2805 & 0.2667 & 0.3329 & 0.3902 & 0.3311 & 0.1583 & 0.6514\\
    \multirow{2}{*}{BL11} & \multirow{2}{*}{Hybrid (BL5 + BL10)} & $\psi_s$ & 0.2777 & 0.2612 & 0.3420 & 0.3869 & 0.3230 & 0.1648 & 0.6540\\
    & & $\psi_j$ & 0.2771 & 0.2615 & 0.3471 & 0.3902 & 0.3246 & 0.1716 & 0.6586\\
    %& & $\psi_j$ & 0.2812 & 0.2699 & 0.3481 & 0.3902 & 0.3377 & 0.1722 & 0.6633\\
    \midrule
    \multicolumn{2}{c}{\textbf{Proposed approaches}} & & & & \\
    \midrule
    \rowcolor{lightgray}
    & FRLM ($\gamma_H=0.8$) & $\psi_l$ & 0.2919 & $0.2810^{\ddagger}$ & $0.3418^{* \dagger \ddagger}$ & 0.3934 & $0.3443^{\ddagger}$ & $0.1616^{* \ddagger}$ & \textbf{0.6786}\\
    %\multirow{2}{*}{} & \multirow{2}{*}{FRLM ($\gamma_H=0.8$)} & $\psi_s$ & 0.2956 & 0.2825 & 0.3507 & 0.4033 & 0.3475 & 0.1688 & 0.6922\\
    \multirow{2}{*}{} & \multirow{2}{*}{FRLM ($\gamma_H=0.8$)} & $\psi_s$ & 0.2956 & 0.2806 & 0.3435 & 0.4033 & 0.3443 & 0.1637 & 0.6922\\
    %& & $\psi_j$ & 0.3075 & 0.2935 & 0.3593 & 0.4131 & 0.3557 & 0.1742 & \textbf{0.7161}\\
    & & $\psi_j$ & $0.3075^{* \dagger \ddagger}$ & $0.2935^{* \dagger \ddagger}$ & $0.3498^{* \dagger \ddagger}$ & 0.4098 & 0.3541 & $0.1687^{* \ddagger}$ & 0.7098\\
    \rowcolor{lightgray}
    %& KDEFRLM & $\psi_l$ & $\textbf{0.2996}^{\dagger \ddagger}$ & \textbf{0.2954} & $\textbf{0.3584}^{* \dagger \ddagger}$ & $\textbf{0.4295}^{\ddagger}$ & \textbf{0.3852} & $\textbf{0.1785}^{* \dagger \ddagger}$ & 0.6553\\
    %& KDEFRLM ($\gamma_H=0.6$) & $\psi_l$ & $\textbf{0.2996}^{\dagger \ddagger}$ & $\textbf{0.2868}^{\dagger \ddagger}$ & $\textbf{0.3490}^{* \dagger \ddagger}$ & $\textbf{0.4295}^{\dagger\ddagger}$ & $\textbf{0.3656}^{\dagger \ddagger}$ & $\textbf{0.1725}^{* \dagger \ddagger}$ & 0.6553\\ % as compared to KDERLM, RLM, BM25
    & KDEFRLM ($\gamma_H=0.6$) & $\psi_l$ & $\textbf{0.2996}^{\dagger \ddagger}$ & $\textbf{0.2868}^{\dagger \ddagger}$ & $\textbf{0.3490}^{* \dagger \ddagger}$ & $\textbf{0.4295}^{\dagger \ddagger}$ & $\textbf{0.3656}^{\dagger \ddagger}$ & $\textbf{0.1725}^{* \dagger \ddagger}$ & 0.6553\\
    %& & $\psi_s$ & $\textbf{0.3135}^{\dagger \ddagger}$ & \textbf{0.2983} & $\textbf{0.3613}^{* \dagger \ddagger}$ & $\textbf{0.4459}^{\ddagger}$ & \textbf{0.3738} & $\textbf{0.1792}^{* \dagger \ddagger}$ & \textbf{0.7068}\\
    \multirow{2}{*}{} & \multirow{2}{*}{KDEFRLM ($\gamma_H=0.7$)} & $\psi_s$ & 0.3079 & 0.2852 & 0.3502 & 0.4361 & 0.3557 & 0.1729 & 0.6648\\
    %& & $\psi_j$ & $\textbf{0.3199}^{\dagger \ddagger}$ & \textbf{0.2987} & $\textbf{0.3655}^{* \dagger \ddagger}$ & $\textbf{0.4525}^{\ddagger}$ & \textbf{0.3770} & $\textbf{0.1832}^{* \dagger \ddagger}$ & 0.7143\\
    & & $\psi_j$ & $\textbf{0.3199}^{*\dagger \ddagger}$ & $\textbf{0.2980}^{*\dagger \ddagger}$ & $\textbf{0.3645}^{* \dagger \ddagger}$ & $\textbf{0.4426}^{* \dagger \ddagger}$ & $\textbf{0.3623}^{*\dagger \ddagger}$ & $\textbf{0.1824}^{* \dagger \ddagger}$ & \textbf{0.7143}\\
    \bottomrule
\end{tabular}
}
%\end{center}
\end{table}



==> tables/resultsTableOutdomain.tex <==
\begin{table}[htb]
\centering
%\small
%\footnotesize
\caption{\hlt{Variations in IR effectiveness} with respect to different choices of pre-trained (out-domain) embedding vectors in comparison to skipgram trained on the target collection (i.e. the result of Table \ref{Table:ResultsCombined2_psi_l} and \ref{Table:ResultsCombined2_psi_j} which is reproduced in this table for convenience).
%- i) \texttt{word2vec} (In-domain), ii) \texttt{word2vec} (Out-domain), iii) \texttt{GloVe} (Out-domain), and iv) \texttt{BERT} (Out-domain), in the performance of KDEFRLM.
}
\label{Table:ResultsOutdomain}
\tabfitpagew{
\begin{tabular}
    %{@{}lllllllllllr@{}}
    {@{}l@{\ \ }l@{\ }l@{\ }l@{\ }l@{\ }l@{\ }lllllr@{}}
    \toprule
    & & & Context & \multicolumn{3}{c}{Graded Evaluation Metrics} & \multicolumn{4}{c}{Binary Evaluation Metrics}\\
    \cmidrule(r){5-7}
    \cmidrule(l){8-11}
    {Method} & Embedding & Domain & $(\psi)$ & nDCG@5 & nDCG@10 & nDCG & P@5 & P@10 & MAP & MRR \\
    \midrule
    \rowcolor{lightgray}
    KDEFRLM & word2vec & In & $\psi_l$ & \textbf{0.2996} & \textbf{0.2868} & 0.3490 & 0.4295 & 0.3656 & 0.1725 & \textbf{0.6553}\\
    \multirow{2}{*}{KDEFRLM} & \multirow{2}{*}{word2vec} & \multirow{2}{*}{In} & $\psi_s$ & 0.3079 & 0.2852 & 0.3502 & 0.4361 & 0.3557 & 0.1729 & 0.6648\\
    & & & $\psi_j$ & \textbf{0.3199} & 0.2980 & 0.3645 & \textbf{0.4426} & 0.3623 & 0.1824 & \textbf{0.7143}\\
    \rowcolor{lightgray}
    KDEFRLM & word2vec & Out & $\psi_l$ & 0.2993 & 0.2840 & 0.3485 & \textbf{0.4328} & 0.3656 & 0.1735 & 0.6367\\
    \multirow{2}{*}{KDEFRLM} & \multirow{2}{*}{word2vec} & \multirow{2}{*}{Out} & $\psi_s$ & 0.2990 & 0.2879 & 0.3539 & 0.4393 & 0.3672 & 0.1758 & 0.6424\\
    & & & $\psi_j$ & 0.3044 & 0.2959 & \textbf{0.3653} & \textbf{0.4426} & 0.3787 & \textbf{0.1844} & 0.6582\\
    \rowcolor{lightgray}
    KDEFRLM & GloVe & Out & $\psi_l$ & 0.2963 & 0.2863 & \textbf{0.3533} & 0.4262 & \textbf{0.3705} & \textbf{0.1750} & 0.6451\\
    \multirow{2}{*}{KDEFRLM} & \multirow{2}{*}{GloVe} & \multirow{2}{*}{Out} & $\psi_s$ & 0.3107 & \textbf{0.3027} & 0.3623 & 0.4361 & \textbf{0.3852} & 0.1802 & 0.6880\\
    & & & $\psi_j$ & 0.3064 & 0.2959 & 0.3638 & 0.4328 & 0.3754 & 0.1815 & 0.6803\\
    \rowcolor{lightgray}
    KDEFRLM & RoBERTa & Out & $\psi_l$ & 0.2971 & 0.2842 & 0.3521 & \textbf{0.4328} & \textbf{0.3705} & 0.1736 & 0.6393\\
    \multirow{2}{*}{KDEFRLM} & \multirow{2}{*}{RoBERTa} & \multirow{2}{*}{Out} & $\psi_s$ & 0.2904 & 0.2894 & 0.3558 & 0.4230 & 0.3754 & 0.1767 & 0.6506\\
    & & & $\psi_j$ & 0.2957 & 0.2855 & 0.3572 & 0.4295 & 0.3721 & 0.1785 & 0.6423\\
    \bottomrule
\end{tabular}
}
%\end{center}
\end{table}


